Language Transformations in the Classroom

Language transformations are algorithms that take a language specification in input, and return the language specification modified. Language transformations are useful for automatically adding features such as subtyping to programming languages (PLs), and for automatically deriving abstract machines. In this paper, we set forth the thesis that teaching programming languages features with the help of language transformations, in addition to the planned material, can be beneficial for students to help them deepen their understanding of the features being taught. We have conducted a study on integrating language transformations into an undergraduate PL course. We describe our study, the material that we have taught, and the exam submitted to students, and we present the results from this study. Although we refrain from drawing general conclusions on the effectiveness of language transformations, this paper offers encouraging data. We also offer this paper to inspire similar studies.

==> eptcsdata.tex <==
\providecommand{\firstpage}{43}
\providecommand{\publicationstatus}{V. Castiglioni and O. Dardha (Eds.): Combined Workshop on \\Expressiveness in Concurrency and Structural Operational Semantics \\ (EXPRESS/SOS 2021)\\
EPTCS 339, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.339.6}{10.4204/EPTCS.339.6}}

